CLIPXPlore: Coupled CLIP and Shape Spaces for 3D Shape Exploration

This paper presents CLIPXPlore, a new framework that leverages a vision-language model to guide the exploration of the 3D shape space. Many recent methods have been developed to encode 3D shapes into a learned latent shape space to enable generative design and modeling. Yet, existing methods lack effective exploration mechanisms, despite the rich information. To this end, we propose to leverage CLIP, a powerful pre-trained vision-language model, to aid the shape-space exploration. Our idea is threefold. First, we couple the CLIP and shape spaces by generating paired CLIP and shape codes through sketch images and training a mapper network to connect the two spaces. Second, to explore the space around a given shape, we formulate a co-optimization strategy to search for the CLIP code that better matches the geometry of the shape. Third, we design three exploration modes, binary-attribute-guided, text-guided, and sketch-guided, to locate suitable exploration trajectories in shape space and induce meaningful changes to the shape. We perform a series of experiments to quantitatively and visually compare CLIPXPlore with different baselines in each of the three exploration modes, showing that CLIPXPlore can produce many meaningful exploration results that cannot be achieved by the existing solutions.

==> tables/abl_quanti.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
            Quantitative analysis of the co-optimization procedure in three exploration scenarios.
            %
            From the FID and Quality Score (QS), the proposed co-optimization can improve the visual quality in all exploration scenarios.
            %
            Further from CLIP-Similarity (CLIP-S) and Matching Score (MS), we can produce shapes fulfilling the given conditions.
 }

		\vspace*{-4mm}
		\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{C{2.0cm}|@{\hspace*{0.3mm}}C{1.5cm}@{\hspace*{0.3mm}}|@{\hspace*{0.3mm}}C{0.8cm}@{\hspace*{0.3mm}}C{0.8cm}@{\hspace*{0.3mm}}C{0.8cm}@{\hspace*{0.3mm}}C{0.8cm}@{\hspace*{0.3mm}}}
			\toprule[1pt]
			% \multirow{1}{Method} 
                Exploration scenario & Method
% 			& \multicolumn{6}{c}{Metrics} \\ \cline{2-7}
			% & \multicolumn{1}{c}{F1-score $\uparrow$}
                & FID $\downarrow$
                & CLIP-S $\uparrow$
			% & \multicolumn{1}{c}{EMD $\downarrow$}
                & QS $\uparrow$
			% & \multicolumn{1}{c}{LFD $\downarrow$} \\ 
                & MS $\uparrow$ \\   \hline
			% & CD & EMD & CD & EMD & CD & EMD \\ \hline
			\multirow{2}{*}{\shortstack[c]{Binary-attribute-guided}} & Without co-opt. & 111.4 & --- & 3.796 & 3.724 \\ 

			& Full pipeline & \textbf{106.9} & --- & \textbf{4.132} & \textbf{4.120} \\ \hline
            \multirow{2}{*}{\shortstack[c]{Text-guided}} & Without co-opt. &  106.4 & 0.842  & 4.224 & 3.644  \\ 
            & Full pipeline & \textbf{100.5} & \textbf{0.886} & \textbf{4.480} & \textbf{4.052} \\
            \hline
            \multirow{2}{*}{\shortstack[c]{Sketch-guided}} & Without co-opt. & 110.2 & 0.961 & 3.808 & 2.904 \\
            & Full pipeline & \textbf{101.4} & \textbf{0.971}  & \textbf{4.636} & \textbf{4.540}\\
			 % Our method & \textbf{0.3431} & \textbf{0.1788} & \textbf{3848.21} \\
			\bottomrule[1pt]
	\end{tabular}}
	%\end{center}
	\label{tab:abl_quanti}
	\vspace{-2mm}
\end{table} 

==> tables/analysis.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
  Comparing our method with various state-of-the-art methods for sketch-based reconstruction. }	%	\begin{center}

		\vspace*{-2mm}
		\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{C{3cm}|C{1cm}C{1cm}C{1cm}}
			\toprule[1pt]
			% \multirow{1}{Method} 
                Method
% 			& \multicolumn{6}{c}{Metrics} \\ \cline{2-7}
			% & \multicolumn{1}{c}{F1-score $\uparrow$}
                & F1-score $\uparrow$
			% & \multicolumn{1}{c}{EMD $\downarrow$}
                & EMD $\downarrow$
			% & \multicolumn{1}{c}{LFD $\downarrow$} \\ 
                & LFD $\downarrow$ \\   \hline
			% & CD & EMD & CD & EMD & CD & EMD \\ \hline
			Sketch2model~\cite{zhang2021sketch2model} & 0.0638 & 0.2309 & 4680.87 \\ 
			sketch2mesh~\cite{guillard2021sketch2mesh} & --- & --- & --- \\
			Sketchsampler~\cite{gao2022sketchsampler} & 0.0719 & 0.1915 & --- \\ \hline
			 Our method & \textbf{0.0867} & \textbf{0.1788} & \textbf{3848.21} \\
			\bottomrule[1pt]
	\end{tabular}}
	%\end{center}
	\label{tab:analysis}
	\vspace{-2mm}
\end{table} 

==> tables/notation.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
  Mathematical symbols employed throughout this paper.  }
  \vspace{-3mm}
	\resizebox{0.85\linewidth}{!}{
		\begin{tabular}{@{\hspace*{1mm}}c@{\hspace*{1mm}}|@{\hspace*{1mm}}c@{\hspace*{1mm}}|@{\hspace*{1mm}}c@{\hspace*{1mm}}}
			\toprule[1pt]
			% \multirow{1}{Method} 
                & Symbol & Description \\   \hline
                \multirow{3}{*}{Input data} & $S_i$ & Training shape \\ 
                & $I_i$ & Rendered sketch image from $S_i$ \\
                & $T_k$ & Shape description text \\ \hline
                \multirow{4}{*}{\shortstack[c]{Latent \\ code}} & $c$   & Latent code in CLIP space \\ 
                & $z$ & Latent code in shape space \\ 
                & $\bar{z}$ & Shape code encoded from input shape \\
                & $\tilde{c}/\tilde{z}$ & Optimized latent code (CLIP/shape space) \\ \hline
                \multirow{4}{*}{\shortstack[c]{Pre-trained \\ model}} & $E_S$ & Shape encoder \\ 
                & $D_S$ & Shape decoder \\ 
                & $E_I$ & CLIP image encoder \\ 
                & $E_T$ & CLIP text encoder \\ 
                % \hline
                % \multirow{3}{*}{\shortstack[c]{Latent \\ direction
                % % \edward{thanks!} \phil{mind the case.. D to d} 
                % }} & $\Delta_{\text{text}}$ & Latent direction 
                % % \phil{mind the case.. D to d} 
                % from a text \\ 
                % & $\Delta_{\text{binary}}$ & Latent direction from a binary attribute \\ 
                % & $\Delta_{\text{sketch}}$ & Latent direction from a sketch image \\ 
			\bottomrule[1pt]
	\end{tabular}
        }
	%\end{center}
	\label{tab:notation}
	\vspace{-4mm}
\end{table} 

==> tables/quan.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
Comparing our method with various state-of-the-art methods for sketch-guided shape exploration.
 %
 From the table, we can see that our manipulated shapes have the best quality for all cases (lowest FID, highest QS and MS) for both the Chair and Table Categories.
 }

		\vspace*{-2mm}
		\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{C{3cm}|C{0.5cm}C{0.5cm}C{0.5cm}|C{0.5cm}C{0.5cm}C{0.5cm}}
			\toprule[1pt]
			% \multirow{2}{Method} 
                Method
			% & \multicolumn{6}{c}{Metrics} \\ \cline{2-7}
			& \multicolumn{3}{c}{Chair}
                % & F1-score $\uparrow$
			& \multicolumn{3}{c}{Table}\\
                % & EMD $\downarrow$
			% & \multicolumn{3}{c}{LFD $\downarrow$} \\ 
                % & LFD $\downarrow$ \\   \hline
			& FID $\downarrow$ & QS $\uparrow$ & MS $\uparrow$ & FID $\downarrow$ & QS $\uparrow$ & MS $\uparrow$ \\ \hline
			Sketch2model~\cite{zhang2021sketch2model} & 168.8 & --- & --- & --- & --- & --- \\ 
			Sketch2mesh~\cite{guillard2021sketch2mesh} & 196.8 & --- & --- & --- & --- & --- \\
			Sketchsampler~\cite{gao2022sketchsampler} & 157.5 & --- & --- & --- & --- & --- \\ \hline

			 Our method & 101.4 & --- & \textbf--- & 147.3 & --- & ---  \\
			\bottomrule[1pt]
	\end{tabular}}
	%\end{center}
	\label{tab:sketch_man_quanti}
	\vspace{-2mm}
\end{table} 

==> tables/recon.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
Comparing our method with various single-viewed reconstruction methods from sketch images.
 %
 From the table, we can see that our reconstructed shapes have the best quality for all cases (highest F1-score, lowest EMD, and lowest LFD) in the Chair Category.}

		\vspace*{-2mm}
		\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{C{3cm}|@{\hspace*{1mm}}c@{\hspace*{2mm}}c@{\hspace*{2mm}}c@{\hspace*{1mm}}}
			\toprule[1pt]
			% \multirow{1}{Method} 
                Method
% 			& \multicolumn{6}{c}{Metrics} \\ \cline{2-7}
			% & \multicolumn{1}{c}{F1-score $\uparrow$}
                & F1-score $\uparrow$
			% & \multicolumn{1}{c}{EMD $\downarrow$}
                & EMD $\downarrow$
			% & \multicolumn{1}{c}{LFD $\downarrow$} \\ 
                & LFD $\downarrow$ \\   \hline
			% & CD & EMD & CD & EMD & CD & EMD \\ \hline
			Sketch2Model~\cite{zhang2021sketch2model} & 0.2832 & 0.2309 & 4680.87 \\ 
			Sketch2Mesh~\cite{guillard2021sketch2mesh} & 0.3293 & 0.1832 & 4192.14 \\
			SketchSampler~\cite{gao2022sketchsampler} & 0.3336 & 0.1915 & 4554.45 \\ \hline
			 Our method & \textbf{0.3431} & \textbf{0.1788} & \textbf{3848.21} \\
			\bottomrule[1pt]
	\end{tabular}}
	%\end{center}
	\label{tab:sketch_recon}
	\vspace{-2mm}
\end{table} 

==> tables/sketch_man_quanti.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
Comparing our method with various state-of-the-art methods for sketch-guided shape exploration.
 %
 From the table, we can see that our manipulated shapes have the best quality for all cases (lowest FID, highest QS and MS) for both the Chair and Table Categories.
 }

		\vspace*{-2mm}
		\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{C{3cm}|C{0.5cm}C{0.5cm}C{0.5cm}|C{0.5cm}C{0.5cm}C{0.5cm}}
			\toprule[1pt]
			% \multirow{2}{Method} 
                Method
			% & \multicolumn{6}{c}{Metrics} \\ \cline{2-7}
			& \multicolumn{3}{c}{Chair}
                % & F1-score $\uparrow$
			& \multicolumn{3}{c}{Table}\\
                % & EMD $\downarrow$
			% & \multicolumn{3}{c}{LFD $\downarrow$} \\ 
                % & LFD $\downarrow$ \\   \hline
			& FID $\downarrow$ & QS $\uparrow$ & MS $\uparrow$ & FID $\downarrow$ & QS $\uparrow$ & MS $\uparrow$ \\ \hline
			Sketch2model~\cite{zhang2021sketch2model} & 168.8 & --- & --- & --- & --- & --- \\ 
			Sketch2mesh~\cite{guillard2021sketch2mesh} & 136.3 & --- & --- & --- & --- & --- \\

			Sketchsampler~\cite{gao2022sketchsampler} & 157.5 & --- & --- & --- & --- & --- \\ \hline
            % Our method (No Optimization) & 106.3038 & 3.60 & 3.30 & 168.3327 & 1.85 & 1.5   \\
			 Our method & 101.4 & --- & \textbf--- & 147.3 & --- & ---  \\
			\bottomrule[1pt]
	\end{tabular}}
	%\end{center}
	\label{tab:sketch_man_quanti}
	\vspace{-2mm}
\end{table} 

==> tables/text_quanti.tex <==
\begin{table}[t]
\scriptsize
	\centering
		\caption{
 \jy{ Comparing our method with various state-of-the-art methods for text-guided shape exploration.
 }}

		\vspace*{-2mm}
		\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{C{3cm}|C{0.5cm}C{0.5cm}C{0.5cm}|C{0.5cm}C{0.5cm}C{0.5cm}}
			\toprule[1pt]

                Method

			& \multicolumn{3}{c}{Chair}

			& \multicolumn{3}{c}{Table}\\

			& FID $\downarrow$ & QS $\uparrow$ & MS $\uparrow$ & FID $\downarrow$ & QS $\uparrow$ & MS $\uparrow$ \\ \hline
			CLIP-Mesh~\cite{mohammad2022clip} & 215.8 & 1.00 & 1.00 & 295.2 & 1 & 1 \\ 
			Text2Mesh~\cite{oscartext2mesh} & 221.5 & 1.40 & 1.40 & 206.8 & 2.5 & 1.5 \\

			TextDeformer~\cite{Gao_2023_SIGGRAPH} & 165.4 & 1.95 & 1.05 & 182.9 & 2.5 & 2.1 \\ \hline

			 Our method & \textbf{100.4} & \textbf{4.35} & \textbf{4.20} & 147.5 & 4.8 & 4.5  \\
			\bottomrule[1pt]
	\end{tabular}}
	%\end{center}
	\label{tab:text_quanti}
	\vspace{-2mm}
\end{table} 
